Bridging the Vision-Brain Gap with an Uncertainty-Aware Blur Prior

Can our brain signals faithfully reflect the original visual stimuli, even including high-frequency details? Although human perceptual and cognitive capacities enable us to process and remember visual information, these abilities are constrained by several factors, such as limited attentional resources and the finite capacity of visual memory. When visual stimuli are processed by human visual system into brain signals, some information is inevitably lost, leading to a discrepancy known as the \textbf{System GAP}. Additionally, perceptual and cognitive dynamics, along with technical noise in signal acquisition, degrade the fidelity of brain signals relative to the visual stimuli, known as the \textbf{Random GAP}. When encoded brain representations are directly aligned with the corresponding pretrained image features, the System GAP and Random GAP between paired data challenge the model, requiring it to bridge these gaps. However, in the context of limited paired data, these gaps are difficult for the model to learn, leading to overfitting and poor generalization to new data. To address these GAPs, we propose a simple yet effective approach called the \textbf{Uncertainty-aware Blur Prior (UBP)}. It estimates the uncertainty within the paired data, reflecting the mismatch between brain signals and visual stimuli. Based on this uncertainty, UBP dynamically blurs the high-frequency details of the original images, reducing the impact of the mismatch and improving alignment. Our method achieves a top-1 accuracy of \textbf{50.9\%} and a top-5 accuracy of \textbf{79.7\%} on the zero-shot brain-to-image retrieval task, surpassing previous state-of-the-art methods by margins of \textbf{13.7\%} and \textbf{9.8\%}, respectively. Code is available at \href{https://github.com/HaitaoWuTJU/Uncertainty-aware-Blur-Prior}{GitHub}.

==> tabs/blurs.tex <==
\begin{table*}[t]
  \centering
  \caption{Top-1 and Top-5 Overall Accuracy (\%) for 200-way Zero-shot Classification on THINGS-EEG}
  \label{tab:var_blur}
  \Huge
\resizebox{\linewidth}{!}{
  \begin{tabular}{lcccccccccccccccccccccc}
    \toprule
    & \multicolumn{2}{c}{Subject 1} & \multicolumn{2}{c}{Subject 2} & \multicolumn{2}{c}{Subject 3} & \multicolumn{2}{c}{Subject 4} & \multicolumn{2}{c}{Subject 5} & \multicolumn{2}{c}{Subject 6} & \multicolumn{2}{c}{Subject 7} & \multicolumn{2}{c}{Subject 8} & \multicolumn{2}{c}{Subject 9} & \multicolumn{2}{c}{Subject 10} & \multicolumn{2}{c}{Avg} \\
    \cmidrule(r){2-3} \cmidrule(r){4-5} \cmidrule(r){6-7} \cmidrule(r){8-9} \cmidrule(r){10-11} \cmidrule(r){12-13} \cmidrule(r){14-15} \cmidrule(r){16-17} \cmidrule(r){18-19} \cmidrule(r){20-21} \cmidrule(r){22-23}
    % \cmidrule{2-23} 
    Method & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 & top-1 & top-5 \\
    \midrule
    Blur kernel 3 &30.1 & 62.4 & 39.6 & 70.0 & 43.5 & 77.5 & 44.4 & 76.2 & 33.5 & 68.8 & 45.5 & 77.9 & 42.1 & 72.3 & 50.5 & 79.9 & 41.1 & 75.0 & 50.1 & 84.8 & 42.1 & 74.5 \\    
    Blur kernel 5 & 33.6 & 65.1 & 40.6 & 74.0 & 42.9 & 78.1 & 46.4 & 79.4 & 35.6 & 70.6 & 48.0 & 78.9 & 43.3 & 73.7 & 56.3 & 81.7 & 42.6 & 71.6 & 55.8 & 86.5 & 44.5 & 76.0\\
    Blur kernel 7 &36.0 & 66.8 & 41.8 & 75.5 & 45.5 & 79.5 & 47.5 & 78.0 & 37.5 & 70.7 & 49.4 & 78.9 & 42.4 & 76.9 & 57.3 & 83.5 & 45.7 & 72.4 & 58.0 & 87.0 & 46.1 & 76.9\\
    Blur kernel 9  &39.0 & 70.1 & 44.8 & 78.0 & 48.2 & 81.4 & 50.6 & 79.9 & 40.1 & 69.9 & 52.9 & 81.0 & 43.6 & 79.3 & 56.5 & 85.3 & 46.9 & 72.9 & 60.5 & 86.3 & 48.3 & 78.4 \\
    Blur kernel 11 &35.8 & 71.0 & 48.9 & 81.5 & 46.8 & 81.6 & 47.7 & 79.4 & 43.4 & 71.1 & 55.5 & 84.5 & 47.7 & 80.0 & 59.3 & 88.1 & 49.1 & 77.0 & 59.0 & 88.9 & 49.3 & 80.3 \\
    Blur kernel 21 & 43.6 & 75.6 & 46.4 & 78.4 & 46.9 & 79.2 & 44.1 & 77.4 & 37.6 & 72.6 & 52.4 & 82.6 & 48.9 & 76.9 & 56.5 & 82.4 & 51.1 & 76.6 & 51.5 & 85.5 & 47.9 & 78.7\\
    Blur kernel 31 & 43.2 & 75.7 & 49.8 & 79.0 & 44.9 & 81.1 & 41.7 & 74.9 & 35.1 & 69.6 & 50.1 & 83.5 & 48.8 & 76.4 & 48.9 & 82.4 & 42.5 & 74.3 & 50.9 & 84.0 & 45.6 & 78.1\\
    Blur kernel 41 &39.4 & 72.6 & 37.1 & 73.1 & 38.2 & 77.1 & 34.1 & 63.9 & 28.6 & 62.6 & 47.4 & 77.8 & 40.9 & 72.6 & 42.7 & 74.6 & 37.4 & 70.2 & 43.0 & 76.6 & 38.9 & 72.1 \\
    
    \bottomrule
  \end{tabular}}
\end{table*}

